Insider Threats in Emerging Mobility-as-a-Service Scenarios

Mobility as a Service (MaaS) applies the everything-as-a-service paradigm of Cloud Computing to transportation: a MaaS provider offers to its users the dynamic composition of solutions of different travel agencies into a single, consistent interface. Traditionally, transits and data on mobility belong to a scattered plethora of operators. Thus, we argue that the economic model of MaaS is that of federations of providers, each trading its resources to coordinate multi-modal solutions for mobility. Such flexibility comes with many security and privacy concerns, of which insider threat is one of the most prominent. In this paper, we follow a tiered structure --- from individual operators to markets of federated MaaS providers --- to classify the potential threats of each tier and propose the appropriate countermeasures, in an effort to mitigate the problems.

==> notes.tex <==
Abbiamo un core che abilitano dei servizi di smart mobility per un singolo operatore.
Questo core lo chiamiamo e-mobility e ti permette di fare info, planning, travelling ecc ecc.
È la nostra attività tecnica di standardizzazione e classificazione dei tipi dati in gioco e dei tipi di servizi
in gioco e relativa definizione degli standard di interfacciamento.

La business intelligence è un altra aggeggio a due strati. La Bi serve anche al singolo operatore così come 
a maggior livello all'operatore.
Il primo layer però è quello che serve all'operatore per sapere come stanno andando le cose, dopodiche nel momento
che si federano più operatori c'è i secondo livello ti intercomunicazione tra gli operatori.
(fare la figura in 3D)

La federation non è soltanto unire più operatori ma anche solamente un tizio che ti da un servizio. Ovvero il core può
anche essere solo un subset.

Nota. Io comunque ho un'unica base di utenti, come mi viene erogato non è importante, ma è cmq un'aspetto di federezaione, 
la vera complicazione sta quando implemento il roaming.

(Andrea) Provare a riscrvere il discorso, c'è una federazione di operatori che accedono alle stesse risorse dati che succede?
Cercare di generalizzarlo non solamente relativo al clearing ma finalizzata all'interoperabilità

(Andrea) Metterci anche la roba di RTSI .. in particolare su Data Provenance

(Andrea) Aggiungere le altre considerazine su data provenance.

(Andrea) Elencare i problemi trovati con Saverio dalla figura.

(Andrea) Leggere articoli di Bishop su Insider Threat.


\section{Note dagli articoli di Bishop}

Per introdurre il concetto di insider threat gli articli di bishop sono ottimi " who guard the guard themselves?"
%
Dobbiamo trattare sia prevention che detection perchè sono due mondi separati e ben distinti!
%
Per la prevention un'ottima base è l'analisi sui nodi che ha fatto Bishop, va estesa col modello di Data Provenance (sarebbe molto figo)
%
Detection bisogna pensare ad un sistema di monitoraggio, scoring, !?!? Deve però tenere conto o di metadata "inviolabili" o di particolari metriche, da cui derivano tutti i discorsi sui falsi positivi e negativi.





\section{Directions in insider threat mitigation}

Many of the described problems are intrinsic to the concepts of cloud, SaaS, and data sharing. 
For this reason, before being able to develop a solution for
data quality and data provenance, there is a need for a preliminary analysis 
of all the metrics of these types of solutions.

\subsection{Data Provenance}

The first thing that we must consider when dealing with services that expose
or elaborate data is to differentiate between data and information.

According to~\cite{cordeiro2008enterprise}, information systems provide data in
a certain business context. When data is used by human beings, it turns
into information, and information finally turns into knowledge by being
interpreted and linked for a given purpose. 
% Regardless of such clear theoretical differentiation between data and
% information, practitioners use the term ``data'' in a broader sense.

As already mentioned, in the context of mobility, verified information is of
paramount importance. \sm supports the provision of different sources of
data along with their associated metadata (e.g., used to verify their
provenance). However, \sm shall also provide techniques, embodied by helper
services, to transform those data into verified information.

Data Provenance verification is a known problem in literature.
Different approaches can be taken to support a solution for the problem of
recognizing the source of a data stream.
Literature agrees~\cite{groth2004protocol} that the requirements for a
provenance management system are:

\begin{itemize}
\item Verifiability: a provenance system should be able to verify a process in
terms of the actors (or services) involved, their actions, and their
relationship with one another.
\item Accountability: an actor (or service) should be accountable for its
actions in a process. Thus, a provenance system should record in a
non-repudiable manner any provenance generated by a service.
\item Reproducibility: a provenance system should be able to repeat a process
and possibly reproduce a process from the provenance stored.
\item Preservation: a provenance system should have the ability to maintain
provenance information for an extended period of time. This is essential for
applications run in an enterprise system.
\item Scalability: given the large amounts of data that an enterprise system
handles, a provenance system needs to be scalable.
\item Generality: a provenance system should be able to record provenance from
a variety of applications.
\item Customizability: a provenance system should allow users to customize it
by setting metadata such as time, events of recording, and the granularity of
provenance.
\end{itemize} 

In a microservice architecture, an application is essentially a collection of workflows.
These workflows can compose many levels of services, each processing and modifying the data
before its final destination. What we need is a way to certify the metadata related 
to a data stream and manage its validity during time and re-elaboration~\cite{tsai2007data}.
Generally literature considers 4 different sets of techniques~\cite{simmhan2005survey}:

\begin{itemize}
\item Subject of Provenance, in which provenance can either be available
explicitly or be deduced indirectly.
\item Representation of Provenance, in which the way provenance is
represented follows from a tradeoff between the cost of recording it and its richness; it is typically implemented either with annotations or with inversion~\cite{bhagwat2005annotation}.
\item Provenance Storage in which the design of metadata is also important to enable scalable storage.
\item Provenance Dissemination where, in order to use provenance, a system
should allow rich and diverse means to access it.
\end{itemize} 

According to works like~\cite{data_provenance_tech1}, this
problem could be solved only with a creation of private and public key system
for data stream certification. A good reference is the system developed
in~\cite{provenance_tech}, describing a cryptographic provenance verification
approach for ensuring data properties and integrity for single hosts.
Specifically, the authors designed and implemented an efficient cryptographic
protocol that enforces keystroke integrity. This kind of protocol can be
integrated as a helper service in \sm. However, public-key schemes are known
for their significant computational load, thus existing techniques may not be
suitable for high-rate, high-volume data sources. Moreover, there could be the
need for an algorithm for the provenance of composed data.

In some cases, data originated from the composition of raw (or otherwise
``lower ranked'') sources should be accompanied by suitable metadata that
allows to verify the provenance of the input values, in a cryptographically
strong way. In the context of \sm, it could be important and useful 
to capture and understand the propagation of data.

In~\cite{zhao2013distributed}, the authors exploit the propagation of
the metadata on the various levels to create a general metadata storage and
management layer for parallel file systems, in which metadata includes both
file operations and provenance metadata.

Also Merkle hash trees could be a
good candidate to build proofs for composed data pieces~\cite{Merkle_tree}.
The combination of metadata propagation with key distribution propagation
management can guarantee a good level of trust in provenance management
systems. Works similar to~\cite{he2015adding} discuss how to support
provenance awareness in spatial data infrastructure and investigates key
issues including provenance modeling, capturing, and sharing that can be
easily used to implement a key propagation system.


\subsection{Data Trustworthiness}

Rating systems are one possible implementation for trustworthiness evaluation
mechanisms. Auditing services, integrated in the \sm platform, attribute
scores to the data-source services based on different criteria. For example,
feedback from users of the data source, or a combination of reputation scores
when the same data can be fed by many sources and cross-checked. Of course,
reputation systems in turn introduce their fair share of
problems~\cite{Reputation, Reputation2, Reputation3,lim2010provenance}. 
An alternative or complementary solutions are anomaly detection services based
on machine learning and pattern recognition~\cite{anomaly}. Then, as cited
for provenance, \sm should automatically compute the trustworthiness score
of data originated from the composition of other sources, based on their
scores.

\subsection{Service Maliciousness}

In principle, the \sm service deployment interface can verify the
correctness of an application before accepting it. In practice, this operation
is very hard to perform. One indicator of correctness is the compliance to a
template of acceptable interfaces for the kind of service the application
provides. However, it is very difficult to define templates strict enough to
allow sensible compliance checks, but general enough to avoid hindering the
deployment of legitimate services. Another way to check correctness is to look
at the actual behavior of the application, as it is common in anti-malware
checks, through static analysis, verifying the code to discover possible
malicious behaviors. These techniques are far from infallible, and their scope
falls much shorter than what is required in our context. Indeed, in this
context a malicious behavior can be a subtle deviation from the correct
calculation~\cite{Malware_Analysis_limits}, which is far more difficult than
the detection of traditional malicious behaviors (e.g., damaging or
self-replicating ones).

A more promising technique is that of dynamic analysis of malware~\cite{dynamic}.
A way to discover a malicious behavior of a service is to implement a mechanism that
could guarantee, in every moment, a reproducibility of the results. Taking
advantage of the data provenance certifications of raw data, and of its
propagation to results, it is possible to implement a reference monitor to
verify the compliance of results to the expected values. In case of conflicts between
the declared results and the actual ones, \sm could discover what has been tampered with:
the source data, or theservice logic. In the first case, this detection can also feed the data
trustworthiness rating system.

\subsection{Service vulnerability to external attacks}
\sm could provide input sanitization, or in general, Intrusion Prevention System / Intrusion Detection System as a service, to protect applications from most of the malicious invocations. Tracing cross-callings between \sm services can
thwart insider attacks aimed at privilege escalation. This can be done by
taking into account the whole set of access control rules before allowing
unauthorized data to leak in or out through a careless application.

% \begin{itemize}
% 	\item Introduzione ai MaaS
%     \item Microservices come sviluppo per i MaaS
%     \item SMall come caso specifico
%     \item Descrizione di Insider Threat nel nostro contesto.
%     \item Panoramica dei problemi di insider threat in una microservice architecture per mobility (MaaS):
% 		\begin{itemize}
% 			\item data provenance
%             \item data trustworthiness
%             \item data maliciuosness
%             \item emerging threats (threats tipiche o del contesto (MaaS) o dei microservizi)
% 		\end{itemize}
        
%     \item Guideline sulle contromisure/mitigaizoni/buone norme ecc
%     \item Sviluppi futuri
%     \item Conclusioni.
% \end{itemize}

